AgroCoT: A Chain-of-Thought Benchmark for Evaluating Reasoning in Vision-Language Models for Agriculture

Recent advancements in Vision-Language Models (VLMs) have significantly impacted various industries. In agriculture, these multimodal capabilities hold great promise for applications such as precision farming, crop monitoring, pest detection, and environmental sustainability. However, while several Visual Question Answering (VQA) datasets and benchmarks have been developed to assess VLM performance, they often fail to effectively evaluate the critical reasoning and problem-solving skills needed in complex agricultural contexts. To address this gap, we introduce AgroCoT, a VQA dataset that integrates Chain-of-Thought (CoT) reasoning, specifically designed to evaluate the reasoning capabilities of VLMs. With 4,759 carefully curated samples, AgroCoT provides a comprehensive and robust evaluation of reasoning abilities, particularly in zero-shot scenarios, focusing on the models' ability to engage in logical reasoning and effective problem-solving. Our evaluation of 30 representative VLMs, including both proprietary and open-source models, reveals a gap in their reasoning capabilities, which underscores the importance of incorporating CoT for assessments. Our dataset is available at https://huggingface.co/datasets/AgroCoT/AgroCoT.

==> table/accuracy.tex <==
\begin{table}[t!]
% \vspace{-0.8cm}
\caption{Accuracy (\%) across different dimensions and models. Abbreviations adopted: QA for Quantitative Analysis; SA for Spatial Analysis; OD for Object Detection; CM for Condition Monitoring; EM for Environmental Management.}
\label{tab:eval_acc}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc}
\Xhline{1.5pt}
\textbf{Model} & \textbf{QA} & \textbf{SA} & \textbf{OD} & \textbf{CM} & \textbf{EM} & \textbf{Overall} \\ 
\Xhline{1.2pt}
\multicolumn{7}{c}{\cellcolor[HTML]{FCE4D6}\textbf{Proprietary Large Vision-Language Models}} \\

Claude-4.5                          & 44.22           & 45.20           & 66.34          & 65.82           & 70.09          & 55.83 \\
Gemini-2.5-pro                      & 42.72           & 49.64           & 66.99          & 71.11           & \textbf{84.15} & 59.14 \\
GPT-4.1                             & 41.75           & 49.02           & 69.38          & 72.11           & 79.46          & 58.96 \\ 
GPT-5                               & \cellcolor[rgb]{.949,  .89,  .988} 50.66  & \textbf{54.26}  & 70.03          & \textbf{76.51}  & 79.68          & \textbf{63.52}  \\

\Xhline{1.2pt}
\multicolumn{7}{c}{\cellcolor[HTML]{FFF2CC}\textbf{Open-Source Large Vision-Language Models}} \\

DeepSeek-VL2                        & 27.62           & 15.18           & 20.41          & 19.51           & 28.79          & 21.56  \\
DeepSeek-VL2-small                  & 34.59           & 16.34           & 30.61          & 27.67           & 30.13          & 27.43  \\
DeepSeek-VL2-tiny                   & 18.01           & 15.89           & 23.56          & 27.34           & 32.14          & 21.87  \\ \hline  
InternVL2-2B                        & 36.80           & 16.78           & 29.21          & 29.20           & 32.14          & 28.31  \\
InternVL2-4B                        & 22.86           & 23.09           & 36.59          & 40.13           & 42.41          & 31.09  \\
InternVL2-8B                        & 38.04           & 39.96           & 55.37          & 48.51           & 50.89          & 45.40  \\
InternVL2-26B                       & 42.81           & 37.21           & 55.70          & 55.46           & 67.41          & 49.00  \\ \hline
InternVL3-2B                        & 34.77           & 33.84           & 41.59          & 30.65           & 43.75          & 35.99  \\
InternVL3-8B                        & 35.48           & 40.76           & 63.08          & 56.01           & 58.26          & 48.75  \\
InternVL3-14B                       & 48.72           & 44.67           & 62.32          & 63.84           & 69.64          & 55.57  \\
InternVL3-38B                       & 46.69           & 45.74           & \textbf{72.64} & 66.48           & 71.43          & 58.13  \\ \hline
LLaVA-NeXT-7B-Mistral               & 27.54           & 14.56           & 22.58          & 24.81           & 39.29          & 23.93  \\
LLaVA-NeXT-8B                       & 38.57           & 23.53           & 35.72          & 41.35           & 38.39          & 34.80  \\
LLaVA-NeXT-13B                      & 10.06           & 13.85           & 12.05          & 15.21           & 17.86          & 13.21  \\
LLaVA-NeXT-34B                      & 49.60           & 29.48           & 50.71          & 39.03           & 46.65          & 42.43  \\ \hline
Qwen2.5-VL-3B-Insturct              & 33.27           & 38.28           & 61.45          & 57.33           & 50.00          & 46.70  \\ 
Qwen2.5-VL-7B-Insturct              & 38.75           & 35.70           & 63.08          & 57.99           & 52.68          & 48.16  \\
Qwen2.5-VL-32B-Insturct             & 33.80           & 15.28           & 16.07          & 17.42           & 23.21          & 21.28  \\ \hline
TinyLLaVA-1.5B                      & 19.51           & 14.56           & 17.59          & 25.58           & 21.21          & 19.27  \\
TinyLLaVA-2B                        & 34.51           & 22.82           & 45.17          & 46.64           & 41.07          & 36.85  \\
TinyLLaVA-3.1B                      & 33.45           & 18.12           & 41.91          & 40.35           & 48.66          & 34.24  \\ \hline
Llama-4-Scout-17B-16E-Instruct      & 40.69           & 40.05           & 61.78          & 65.05           & 64.73          & 52.06  \\ 

\Xhline{1.5pt}
\end{tabular}
}
\vspace{-1cm}
\end{table}


==> table/benchmark_comparison.tex <==
\begin{table}
\caption{Comparison of AgriCoT with existing agriculture datasets or benchmark. CoT shows whether the dataset contains Chain-of-Thought reasoning. Abbreviations adopted: \#Q for the number of questions; MCQ for Multiple Choice Questions; TFQ for True-or-False Questions; OEQ for Open-Ended Questions; LFQ for Long-From Question-answering; Conv for Conversational multi-turn interactions. AgriCoT is the only dataset in the agricultural domain that contains CoT.}
\label{tab:benchmark_comparison}
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccc}
        \Xhline{1.2pt}
        \textbf{Dataset}                                  & \textbf{\#Q}     & \textbf{Answer Type}     & \textbf{Multimodal}    & \textbf{Multi-view}   & \textbf{CoT}   \\
        \Xhline{1.2pt}        
        CROP~\cite{zhang2024empowering}                   & 5,045            & MCQ                      & \XSolidBrush           & \XSolidBrush            & \XSolidBrush  \\
        CDDM~\cite{liu2024multimodal}                     & 1 million        & TFQ, OEQ                 & \Checkmark             & \XSolidBrush            & \XSolidBrush  \\ 
        AgroInstruct~\cite{awais2025agrogpt}              & 70 K             & TFQ, OEQ                 & \Checkmark             & \XSolidBrush            & \XSolidBrush  \\
        MIRAGE~\cite{dongre2025mirage}                    & 41 K             & LFQ, Conv                & \Checkmark             & \XSolidBrush            & \XSolidBrush  \\
        AGMMU~\cite{gaubaagmmu}                           & 1,492            & MCQ, OEQ                 & \Checkmark             & \XSolidBrush            & \XSolidBrush  \\
        AgroBench~\cite{shinoda2025agrobench}             & 4,342            & MCQ                      & \Checkmark             & \XSolidBrush            & \XSolidBrush  \\
        AgriBench-VL-4K~\cite{yang2025agrigpt}            & 3,876            & MCQ, OEQ                 & \Checkmark             & \XSolidBrush            & \XSolidBrush  \\
        AgroMind~\cite{li2025can}                         & 28,482           & MCQ, TFQ, OEQ            & \Checkmark             & \Checkmark              & \XSolidBrush  \\ \hline
        \rowcolor{green!20}
        AgriCoT (Ours)                                    & 4,759            & MCQ, TFQ, OEQ            & \Checkmark             & \Checkmark              & \Checkmark    \\ 
        \Xhline{1.2pt}
    \end{tabular}
}
\vspace{-1.5em}
\end{table}



==> table/bertscore.tex <==
\begin{table}
\caption{BERTScore-f (\%) across different dimensions and models. Abbreviations adopted: QA for Quantitative Analysis; SA for Spatial Analysis; OD for Object Detection; CM for Condition Monitoring; EM for Environmental Management. ``-'' indicates that the model is unable to output a normal CoT reasoning, resulting in a negative BERTScore.}
\label{tab:bertscore}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc}
\Xhline{1.5pt}
\textbf{Model} & \textbf{QA} & \textbf{SA} & \textbf{OD} & \textbf{CM} & \textbf{EM} & \textbf{Overall} \\ 
\Xhline{1.2pt}
\multicolumn{7}{c}{\cellcolor[HTML]{FCE4D6}\textbf{Proprietary Large Vision-Language Models}} \\

Claude-4.5                          & 48.44          & 43.89          & 45.85          & 45.35          & 44.15          & 45.74 \\
Gemini-2.5-pro                      & 35.41          & 30.95          & 32.26          & 33.02          & 32.28          & 32.88 \\
GPT-4.1                             & \textbf{52.11} & \textbf{48.43} & \textbf{48.28} & \textbf{49.11} & \textbf{45.66} & \textbf{49.18} \\ 
GPT-5                               & 30.42          & 29.55          & 26.21          & 27.92          & 28.83          & 28.69 \\ 

\Xhline{1.2pt}
\multicolumn{7}{c}{\cellcolor[HTML]{FFF2CC}\textbf{Open-Source Large Vision-Language Models}} \\

DeepSeek-VL2                        & -              & -              & -              & -              & -              & -       \\
DeepSeek-VL2-small                  & -              & -              & -              & -              & -              & -       \\
DeepSeek-VL2-tiny                   & 7.81           & -              & -              & -              & -              & -       \\  \hline
InternVL2-2B                        & 25.68          & 25.52          & 24.49          & 23.78          & 20.07          & 24.46   \\
InternVL2-4B                        & 39.35          & 34.63          & 30.67          & 34.07          & 31.66          & 34.60   \\
InternVL2-8B                        & 38.72          & 38.04          & 36.41          & 35.95          & 35.80          & 37.24   \\
InternVL2-26B                       & 38.74          & 41.24          & 35.52          & 37.43          & 35.73          & 38.15   \\  \hline
InternVL3-2B                        & 37.54          & 25.88          & 26.21          & 28.25          & 30.67          & 29.81   \\
InternVL3-8B                        & 35.05          & 27.60          & 30.94          & 28.35          & 28.83          & 30.41   \\
InternVL3-14B                       & 38.44          & 27.34          & 34.51          & 33.71          & 32.86          & 33.39   \\
InternVL3-38B                       & 40.51          & 36.89          & 36.50          & 35.17          & 35.34          & 37.22   \\  \hline
LLaVA-NeXT-7B-Mistral               & 29.52          & 27.74          & 24.81          & 27.85          & 28.29          & 27.67   \\
LLaVA-NeXT-8B                       & 34.54          & 35.48          & 29.77          & 33.81          & 30.99          & 33.31   \\
LLaVA-NeXT-13B                      & 10.55          & 19.86          & 17.14          & 16.62          & 17.45          & 16.09   \\
LLaVA-NeXT-34B                      & 26.42          & 32.48          & 31.82          & 29.76          & 32.24          & 30.27   \\  \hline
Qwen2.5-VL-3B-Insturct              & 31.65          & 27.49          & 24.75          & 24.43          & 26.16          & 27.23   \\
Qwen2.5-VL-7B-Insturct              & 34.09          & 30.63          & 25.82          & 26.76          & 25.94          & 29.28   \\
Qwen2.5-VL-32B-Insturct             & 33.13          & 30.11          & 28.36          & 27.62          & 30.38          & 29.54   \\  \hline
TinyLLaVA-1.5B                      &  9.28          & -              & -              & -              & -              & -       \\
TinyLLaVA-2B                        & -              & -              & -              & -              & -              & -       \\
TinyLLaVA-3.1B                      &  4.76          &  0.93          & -              & -              &  2.41          &  0.37   \\  \hline
Llama-4-Scout-17B-16E-Instruct      & 43.63          & 36.87          & 40.31          & 41.18          & 38.65          & 40.29   \\
\Xhline{1.5pt}
\end{tabular}
}
% \vspace{-3mm}
\end{table}

==> table/rouge.tex <==
\begin{table}
\caption{ROUGE-L-f (\%) across different dimensions and models. Abbreviations adopted: QA for Quantitative Analysis; SA for Spatial Analysis; OD for Object Detection; CM for Condition Monitoring; EM for Environmental Management.}
\label{tab:rouge}
% \centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc}
\Xhline{1.5pt}
\textbf{Model} & \textbf{QA} & \textbf{SA} & \textbf{OD} & \textbf{CM} & \textbf{EM} & \textbf{Overall} \\ 
\Xhline{1.2pt}
\multicolumn{7}{c}{\cellcolor[HTML]{FCE4D6}\textbf{Proprietary Large Vision-Language Models}} \\                                                                                                                                                                          
Claude-4.5                         & 47.09          & 41.70          & 45.22          & 45.95           & 44.77          & 44.92  \\
Gemini-2.5-pro                     & 36.39          & 32.65          & 35.16          & 36.77           & 36.21          & 35.27  \\
GPT-4.1                            & \textbf{50.99} & \textbf{45.93} & \textbf{47.25} & \textbf{49.79}  & \textbf{46.62} & \textbf{48.31}  \\ 
GPT-5                              & 30.46          & 27.65          & 27.76          & 29.27           & 28.46          & 28.78  \\ 

\Xhline{1.2pt}
\multicolumn{7}{c}{\cellcolor[HTML]{FFF2CC}\textbf{Open-Source Large Vision-Language Models}} \\

DeepSeek-VL2                       & 16.18          &  8.63          & 11.92           & 11.09          &  6.52          & 11.47    \\
DeepSeek-VL2-small                 & 16.92          &  7.87          & 12.31           & 14.86          & 11.93          & 12.83    \\
DeepSeek-VL2-tiny                  & 16.79          &  7.24          & 12.55           & 10.38          &  5.42          & 11.15    \\  \hline
InternVL2-2B                       & 29.02          & 28.64          & 29.68           & 29.02          & 27.89          & 28.95    \\
InternVL2-4B                       & 40.25          & 34.98          & 33.95           & 36.71          & 34.62          & 36.40    \\
InternVL2-8B                       & 38.08          & 38.67          & 37.03           & 38.45          & 38.35          & 38.11    \\
InternVL2-26B                      & 38.62          & 40.49          & 37.72           & 38.81          & 37.47          & 38.82    \\  \hline
InternVL3-2B                       & 39.73          & 33.70          & 34.62           & 34.72          & 37.04          & 35.93    \\
InternVL3-8B                       & 42.63          & 39.19          & 38.81           & 39.46          & 40.71          & 40.18    \\
InternVL3-14B                      & 46.23          & 38.08          & 42.01           & 40.98          & 40.82          & 41.77    \\
InternVL3-38B                      & 44.29          & 38.50          & 39.15           & 39.17          & 38.95          & 40.25    \\  \hline
LLaVA-NeXT-7B-Mistral              & 32.36          & 31.89          & 30.79           & 32.87          & 31.05          & 31.90    \\
LLaVA-NeXT-8B                      & 34.56          & 37.15          & 34.05           & 35.91          & 33.81          & 35.29    \\
LLaVA-NeXT-13B                     & 23.45          & 26.92          & 25.79           & 26.95          & 25.99          & 25.74    \\
LLaVA-NeXT-34B                     & 32.13          & 34.04          & 33.12           & 33.19          & 33.98          & 33.20    \\  \hline
Qwen2.5-VL-3B-Insturct             & 32.45          & 30.70          & 29.54           & 29.66          & 31.80          & 30.80    \\
Qwen2.5-VL-7B-Insturct             & 36.28          & 33.38          & 31.89           & 32.91          & 31.30          & 35.50    \\
Qwen2.5-VL-32B-Insturct            & 36.73          & 33.33          & 33.85           & 35.05          & 36.11          & 34.90    \\  \hline
TinyLLaVA-1.5B                     & 18.29          &  7.72          & 11.16           &  8.60          & 10.32          & 11.49    \\
TinyLLaVA-2B                       &  3.52          &  5.71          &  5.28           &  3.46          &  4.85          &  4.54    \\
TinyLLaVA-3.1B                     & 16.06          & 12.65          & 11.58           & 10.40          & 13.51          & 12.92    \\  \hline
Llama-4-Scout-17B-16E-Instruct     & 44.90          & 37.88          & 41.35           & 43.40          & 41.34          & 41.78    \\ 
\Xhline{1.5pt}
\end{tabular}%
}
% \vspace{-3mm}
\end{table}
